IconQA: A New Benchmark for Abstract Diagram Understanding and Visual Language Reasoning

Current visual question answering (VQA) tasks mainly consider answering human-annotated questions for natural images. However, aside from natural images, abstract diagrams with semantic richness are still understudied in visual understanding and reasoning research. In this work, we introduce a new challenge of Icon Question Answering (IconQA) with the goal of answering a question in an icon image context. We release IconQA, a large-scale dataset that consists of 107,439 questions and three sub-tasks: multi-image-choice, multi-text-choice, and filling-in-the-blank. The IconQA dataset is inspired by real-world diagram word problems that highlight the importance of abstract diagram understanding and comprehensive cognitive reasoning. Thus, IconQA requires not only perception skills like object recognition and text understanding, but also diverse cognitive reasoning skills, such as geometric reasoning, commonsense reasoning, and arithmetic reasoning. To facilitate potential IconQA models to learn semantic representations for icon images, we further release an icon dataset Icon645 which contains 645,687 colored icons on 377 classes. We conduct extensive user studies and blind experiments and reproduce a wide range of advanced VQA methods to benchmark the IconQA task. Also, we develop a strong IconQA baseline Patch-TRM that applies a pyramid cross-modal Transformer with input diagram embeddings pre-trained on the icon dataset. IconQA and Icon645 are available at https://iconqa.github.io.

==> NeurIPS 2021 Track on Datasets_IconQA/cards/card_icon645.tex <==
\sffamily
{
\fbox{%
    \begin{tabular}{@{}p{\NFwidth}@{}}
    
    % Top Matter    
    % \NFtitle\\
    \multicolumn{1}{c}{\huge\bfseries Icon645 Dataset Facts}\\
    \NFrule
    % \NFtext{\textbf{Website} iconqa.github.io}\\
    \NFelement{Website}{}{\url{https://iconqa.github.io}}\\
    % Motivation Section
    \NFRULE
    \NFline{Metadata}\\
    \NFrule
    \NFelement{Classes}{}{377}\\
    \NFelement{Instances}{}{645,687}\\
    \NFelement{Format}{}{.png}\\
    \NFelement{Image Sizes}{}{64$\times$ 64 - 256 $\times$ 256}\\
    \NFelement{License}{}{CC BY-NC-SA}\\
    \NFelement{Original Use Case}{}{Training visual encoder}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Composition Section
    \NFRule
    \NFline{Composition}\\
    \NFrule
    \NFelement{Sample or Complete}{}{Sample from \text{flaticon.com}}\\
    \NFelement{Missing Data}{}{No data is missing}\\
    %\NFelement{Sensitive Information }{}{Info}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Collection Process Section
    \NFRule
    \NFline{Collection}\\
    \NFrule
    \NFelement{Sampling Strategy}{}{See the main paper}\\
    % \NFelement{Ethical Review}{}{}\\
    \NFelement{Author Consent}{}{None needed}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Cleaning / Labeling Section
    \NFRule
    \NFline{Cleaning and Labeling}\\
    \NFrule
    \NFelement{Cleaning Done}{}{Repetitions and redundancies removed}\\
    \NFelement{Labeling Done}{}{Yes}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Uses / Distribution Section
    \NFRule
    \NFline{Uses and Distribution}\\
    \NFrule
    \NFelement{Notable Uses}{}{Pre-training abstract icon image encoder}\\
    \NFelement{Other Uses}{}{Abstract image classification, transfer learning}\\
    \NFelement{Original Distribution}{}{Check dataset website}\\
    %\NFelement{Replicate Distribution}{}{Info}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Maintenance and Evolution Section
    \NFRule
    \NFline{Maintenance and Evolution}\\
    \NFrule
    \NFelement{Corrections or Erratum}{}{None as of now}\\
    \NFelement{Methods to Extend}{}{Contact the author}\\
    %\NFelement{Replicate Maintainers}{}{Maintainer}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    \NFRULE
    \end{tabular}}
\par} % to end centering

==> NeurIPS 2021 Track on Datasets_IconQA/cards/card_iconqa.tex <==
\sffamily
{
\fbox{%
    \begin{tabular}{@{}p{\NFwidth}@{}}
    
    % Top Matter
    % \NFtitle\\
    \multicolumn{1}{c}{\huge\bfseries IconQA Dataset Facts}\\
    \NFrule
    % \NFtext{\textbf{Website} iconqa.github.io}\\
    \NFelement{Website}{}{ \url{https://iconqa.github.io}}\\
    
    % Motivation Section
    \NFRULE
    \NFline{Metadata}\\
    \NFrule
    \NFelement{Instances}{}{107,439}\\
    \NFelement{Format}{}{.png, .json}\\
    \NFelement{License}{}{CC BY-NC-SA}\\
    \NFelement{Original Use Case}{}{Training VQA systems}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Composition Section
    \NFRule
    \NFline{Composition}\\
    \NFrule
    \NFelement{Sample or Complete}{}{Sample from \text{ixl.com}}\\
    \NFelement{Missing Data}{}{No data is missing}\\
    %\NFelement{Sensitive Information }{}{Info}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Collection Process Section
    \NFRule
    \NFline{Collection}\\
    \NFrule
    \NFelement{Sampling Strategy}{}{See the main paper}\\
    % \NFelement{Ethical Review}{}{}\\
    \NFelement{Author Consent}{}{None needed}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Cleaning / Labeling Section
    \NFRule
    \NFline{Cleaning and Labeling}\\
    \NFrule
    \NFelement{Cleaning Done}{}{Repetitions and redundancies removed}\\
    \NFelement{Labeling Done}{}{Yes}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Uses / Distribution Section
    \NFRule
    \NFline{Uses and Distribution}\\
    \NFrule
    \NFelement{Notable Uses}{}{Training VQA systems}\\
    % \NFelement{Other Uses}{}{Probably None}\\
    \NFelement{Original Distribution}{}{Check dataset website}\\
    %\NFelement{Replicate Distribution}{}{Info}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    % Maintenance and Evolution Section
    \NFRule
    \NFline{Maintenance and Evolution}\\
    \NFrule
    \NFelement{Corrections or Erratum}{}{None as of now}\\
    \NFelement{Methods to Extend}{}{Contact the author}\\
    %\NFelement{Replicate Maintainers}{}{Maintainer}\\
    %\NFelement{Additional Field}{}{Info}\\
    
    \NFRULE
    \NFline{Breakdown \hfill\% of Example}\\
    \NFrule
    \NFelement{multi-image-choice}{57,672\,items}{53.7\%}\\
    \NFrule
    \NFelement{multi-text-choice}{31,578\,items}{29.4\%}\\
    \NFrule
    \NFelement{fill-in-the-blank}{18,189\,items}{16.9\%}\\
    \NFrule
    %\NFelement{Another}{count}{XX\%}\\
    %\NFrule
    \end{tabular}}
\par} % to end centering
